Clustering in networks with the collapsed Stochastic Block Model

An efficient MCMC algorithm is presented to cluster the nodes of a network such that nodes with similar role in the network are clustered together. This is known as block-modelling or block-clustering. The model is the stochastic blockmodel (SBM) with block parameters integrated out. The resulting marginal distribution defines a posterior over the number of clusters and cluster memberships. Sampling from this posterior is simpler than from the original SBM as transdimensional MCMC can be avoided. The algorithm is based on the allocation sampler. It requires a prior to be placed on the number of clusters, thereby allowing the number of clusters to be directly estimated by the algorithm, rather than being given as an input parameter. Synthetic and real data are used to test the speed and accuracy of the model and algorithm, including the ability to estimate the number of clusters. The algorithm can scale to networks with up to ten thousand nodes and tens of millions of edges.

==> extending.tex <==
\section{Extensions}
\label{SECextending}

% \emph{I should double-check some of the claims in this section - Aaron.}

In this paper we have applied parameter collapsing to a subset of  the models presented in \cite{Nowicki-01}.
It is possible to apply this strategy to their full range of models in a similar fashion to that described here, allowing for $K$ to be estimated in this fully Bayesian approach.
For example, it is possible to allow for missing data, and also to allow for a broader `alphabet' as mentioned previously.

It is also possible to conceive of a hierarchical extension to the SBM which is suitable for collapsing.
At the `top-level', the standard SBM models connections between clusters.  Next, the internal connections within each cluster are again modelled as an SBM producing a set of sub-clusters within each cluster.
This process can be applied recursively to any depth, and the
resulting ``clustering'' can be represented as a tree.
As far as we are aware, this generalized model has not appeared in the literature.
However, it is interesting that two specializations of this model have. In \cite{BaderParkBinaryTree}, an SBM is used at the top level to model
the between-cluster interactions, and each cluster is then modelled
as a \emph{binary} tree.
This is a specialization with the restriction that the number
of subclusters (and sub-sub-clusters etc) is fixed at $K=2$
at every level except the top level.  Also, in \cite{ClausetHierNetworks} a further restriction is presented, where
even the ``top-level'' K is fixed at 2.





==> reviewers.tex <==
\break
\newenvironment{myindentpar}[1]%
     {\begin{list}{}%
             {\setlength{\leftmargin}{#1}}%
             \item[]%
     }
     {\end{list}}
\definecolor{dark-green}{RGB}{0,80,0}
\definecolor{light-gray}{gray}{0.5}
\newcommand{\red}[1]{{\color{red} \begin{myindentpar}{2cm}#1\end{myindentpar}}}
\newcommand{\blue}[1]{{\color{blue} \begin{myindentpar}{2cm}#1\end{myindentpar}}}
\newcommand{\green}[1]{{\color{dark-green} \begin{myindentpar}{2cm}#1\end{myindentpar}}}
\newcommand{\amd}{\emph{AMcD}}
\section{Reviewers' comments}

We would like to thank the reviewers for their useful and interesting comments.
In this response, we have copied the reviewers' comments in the original order,
indented and coloured green,
and we will make our detailed responses at the appropriate place below.
However, we will make some brief overall comments first.

In this review copy, we have arranged for lines numbers to appear
in the left margin, and we will refer to those line numbers in some of our responses.

The title has been changed, as suggested by Reviewer \#2.  It's now
``Improved Bayesian Inference for the Stochastic Block Model with application to large networks''

The overall structure has changed in some important ways.  The order of the presentation
is the same, but some subsections have been added or removed or changed significantly.
More detailed responses will be made later.
\begin{itemize}
	\item Section 1: The introduction. Now includes some extra references.
	\item Section 2: Define the SBM.  We have nothing novel here, we just define the model based on existing literature.
	\item Section 3: The term `collapsing' is introduced, and our marginalization is derived.
	\item Section 4: Related estimation procedures: Discuss algorithms already in the literature, focussing exclusively on the SBM. Also includes a completely rewritten subsection on the various approaches to model selection for the SBM.
	\item Section 5: Estimation:  Our algorithm.
	\item Section 6: Synthetic evaluation: Includes some new experiments.
	\item Section 7: Our analysis of the summer school survey network.
	\item Section 8: Conclusion: rewritten to account for the changes that have been made.
\end{itemize}


\subsection{Reviewer 1}

\green{The authors propose an interesting approach for the stochastic block model that I do recommend for publication.
Contrary to existing techniques which rely on approximations (variational decompositions for instance), they derive exact quantities, using common
conjugate priors such as Beta and Dirichlet priors. These collapsed quantities are maximized for inference using a MCMC algorithm, related to the
allocation sampler which was proposed in the context of a more standard Gaussian mixture model.
Four moves (Metropolis, Gibbs sampling, Metropolis-Hastings, absorb-eject move) are proposed to search over
the space of possible clusterings and number of classes.
I see three main advantages of their work compared to existing strategies for the stochastic block model :
Usually, existing methods are run several times for various  values of the number of classes K, a model selection criterion is computed,
and K is chosen such that the corresponding criterion is maximized. Here, because a Poisson prior distribution is considered and thanks
to the MCMC moves, K is estimated automatically from the data.
Second, the authors maximize an exact collapsed distribution and I expect this to lead to better results than inference strategies based on
variational approximations. Finally, the experiment section illustrates that their algorithm is rather fast, making it possible to use
the stochastic block model on large networks (few thousand nodes) while the algorithm of Nowicki \& Snijders can be only be used for networks
with a few hundred of nodes for instance. Moreover, the authors made their code publicly available as well as the original data set they use in the experiment section.
Some more specific comments below :}

\green{In the Introduction :}

\green{* I agree with the authors that the community finding problem should be distinguish with the more general problem of block modeling.}

Thanks for the accurate summary of the paper.

\green{* Some common references are missing. In particular, I would like the authors to add references to community detection algorithms which
are highly used for graph clustering. I understand that in the paper the authors consider methods based on probabilistic models,
however, I feel these algorithms represent an important part of the literature and should be mentioned.
I suggest that the authors describe in a few sentences the modularity criterion and one or two strategies to optimize it.
The following references could be added:

-\cite{NewmanGirvan} Newman and Girvan. Finding and evaluating community structure in networks. Physical Review. 2004

-\cite{girvan-2002} Girvan and Newman. Community structure in social and biological networks. PNAS. 2002

- \cite{NewmanFastishMod} Newman. Fast algorithm for detecting community structure in networks. Physical Review. 2004

References (and a bit of description) to three common probabilistic models for graph should also be added :

- \cite{HandcockRafteryTantrum} The latent position cluster model (LPCM) :  Handcock, Raftery, and Tantrum. Model based clustering for social networks. Journal of the royal statistical society. 2007.

- \cite{HoffLatentSpace} LPCM generalizes the work the latent space model : Hoff and Raftery, and Handcock. Latent space approaches to social network analysis. Journal of the royal statistical society. 2002.

- \cite{Airoldi2008MMSB} The mixed membership model :  Airoldi, Blei, Fienberg, Xing. Mixed membership stochastic block models. 2008
}

These references have been added.  Near the end of Section~1(`Introduction'), lines 57, we have listed a wide variety of alternative
approaches to clustering the nodes of a network, other than those that are directly based on the SBM.
This includes statistical approaches and non-statistical approaches.
However, we have not given any further details or description of these methods, to save space;
the reader is directed to Fortunato's review \citep{fortunato-2010} if they would like a more comprehensive summary.
The models and methods that are based on the SBM are discussed in later sections.

\green{
* Page 3, section 2. When describing the stochastic block model, I suggest the authors first mention that the model is sometimes described
in a frequentist setting as in Daudin et al (2008) and that they are here considering a Bayesian framework as in (Nowiki and Snijders, 2001) and Latouche et al (2012).
}

We discuss this at the bottom of page 4, just before Subsection~2.1(`DataModelVariations') at lines 137 to 145, and also in Section~4(`RelatedEstimationProcedures') at lines 258 to 268,
noting the practical difference between the frequentist and Bayesian approach.
The frequentist approaches use a point estimate for the parameters, specifically the MLE, whereas
the Bayesian approach considers a full distribution based on a prior.
We avoid any philosophy, our goal is to provide the practical guidance on what is different
from an algorithmic point of view.

\green{
* Page 3 : "Section 4," -$>$ remove ","

* Page 5 : "rather then requiring" -$>$ "rather than requiring"

* Page 10 : "alternatively, the an" -$>$ "alternatively, an"
}
These typographical errors, and others we had missed, have been corrected throughout the paper.

\green{
* Page 4 : sometimes the authors forget to add comma or point at the end of the formulae. First formulae : comma missing. Third formulae : point missing.
Check the rest of the paper, especially the appendix section.
* Page 11 : first formulae : point missing
}

This was an issue right throughout the paper.  Every formula has now been checked and edited.

\break
\green{
* Page 9 : the equation should be removed or given directly in the text or being introduced first. A simple : "$P(x|K)$ is given by : ." might be sufficient.
}
Done. Now on page 12, line 313. This is Subsection~4.1(`Model Selection'). An expression for $\mathrm{P}(x|K)$, based on a suitable summation and integration, is now given in a more direct manner.

\green{
* Page 7, section 4 : When the authors mention the constraints on pi that Zanghi et al (2008) used, they could refer to the work of Hofman and Wiggins (2008) which is very similar.
}
This reference \cite{HofmanBayesNetworkModularity} has been added to Section~4(`Related Estimation Procedures') line 270.

\green{
When they first introduce BIC ("BIC is used to ."), the authors should recall that in the case of the stochastic block model,
BIC is not tractable (because the likelihood is not tractable).
Also, for the rest of the section, do not describe BIC as if it was a model selection criterion among others that could be used to estimate K.
Again, it is not tractable  in the case of the stochastic block model.
}
This is a good point. The subsection~4.1(` Model selection') has been rewritten.
We focus on issues more directly related to the SBM, and have removed much of the more general discussion.
We have mentioned the BIC, but we have shortened our discussion of it;
even though it is not tractable in practice, it may be interesting to briefly discuss
the \emph{integrated likelihood}, $\mathrm{P}(x|K)$, which the BIC attempts to approximate.
This allows us to discuss how our allocation sampler, and the $ILvb$ of \cite{LatoucheILvbStatMod},
may also be used to approximate the \emph{integrated likelihood}.

\green{

* Page 17 : when the authors first mention the Erdos-Renyi model, they could recall that this model corresponds to a random graph model with no
block structure.

* same page : "as expected, this decreases as delta increases. " -$>$ explain why.
}
On page 22, line 605, We now state that, as delta tends to 0.5 , the network approaches the Erdos-Renyi network and therefore that
the accuracy decreases due to the lack of block structure.

\green{
Experiment section : I enjoyed reading the experiment section which, through a series of analysis of both toy data and real data sets, illustrates the capacity of the approach to estimate K and retrieve the clustering structure. However, the authors could easily do a little more to demonstrate the utility of their approach : I would like to see how the criterion of Latouche et al (2012) performs against the proposed approach.
}
We have included two new experiments based on the experiments of Latouche et al (2012) \cite{LatoucheILvbStatMod}.
In subsection~6.2(`Estimating K in community-structure networks') we copied the \emph{community-structure} experiments
exactly from their paper, using their software, and compared the answer with that from our method.
In subsection~6.3(`Synthetic SBM networks') we modified their data-generation software to generated data more strictly from the SBM,
and performed the same sort of experiments again.
We used larger networks, with larger $K$, in this second set of experiments.











\subsection{Reviewer 2}
\green{
The paper describes a bayesian MCMC inference for The Stochastic Block Model. The method is a significant  improvement to published work on the same problem. The proposed MCMC procedure allows to deal with quite larger data sets than the old one, which was limited to networks with 200 nodes. Moreover it gives a procedure to estimate the number of groups. Therefore the proposed algorithm is a real progress, which deserves publication. However it suffers from its poor presentation which has to be significantly improved.

Major comments
}
 \dots

\green{
1. The presentation is confusing because there is no clear distinction between the model and the algorithm used to estimate the parameters.
}
We have changed the structure as described at the top of our response above.
The model is described in section 2, our collapsing/marginalization in section 3, and our algorithm in section 5.
Alternative SBM algorithms in the literature have been discussed in section 4.

\green{
The authors claimed that their model is an extension of the Stochastic Block Model. But this is not true. The model is  exactly the SBM.
}
Thanks for the reference to the Mariadassou work \cite{MariadassouWeightedSBM}.
We were not aware that the Poisson edge-weight model was not new, and therefore we thought that we had extended the model.
We have made a number of changes throughout the paper to correct for this.

\green{
The "collapsing" procedure is only the computation of a marginal distribution in the Bayesian version of the SBM.
}
Agreed.
It is a technique to simplify the representation of the posterior which allows for simpler mathematics and simpler algorithms,
and hence it is more of an `algorithmic' issue than a `modelling' issue.
We no longer refer to this as an `extension' - it does not change the model
and it does not change the results for $(z,K|x)$ that we extract from the posterior.

\green{
The extension to weighted networks (Poisson and Gaussian) have been already published (see for example M. Mariadassou, S. Robin, and C. Vacher, Uncovering structure in valued graphs: A variational approach, Ann. Appl. Statist. 4(2) (2010), pp. 715-742).
}
Agreed. Discussed above.

\green {
Therefore the model is not new, but the MCMC algorithm is. The authors have to correct this confusion in many places in the paper. For example, the title should be modified. I suggest "New MCMC Bayesian Inference for the Stochastic Block Model", but the authors may find another title in the same spirit. The words "we extend the SBM model"
should be suppressed everywhere in the paper.
}
We now have a new title - `Improved Bayesian Inference for the Stochastic Block Model with application to large networks'.
The word `extend' has been suppressed.

\green{
2. There is some dispersion in the presentation and the authors should have a better focus and shorten the paper.
The paper should be reorganized in a more logical way: Introduction, model, published methods (frequentist and bayesian with more focus on bayesian ones) and algorithms for estimating parameters, the proposed MCMC algorithm incuding the estimation of K and label switching, Simulations, Analysis of a real data set and conclusion.
}
Done - that's the structure now.

\green{
 2.1 The presentation of the alternative published methods has to be modified: some of them are out of the scope, others are lacking.

 The subject is the SBM, so it is not usefull to refer to other models in the section "Related probabilistic models". This section is confusing because of the confusion between models and algorithms.
 The authors must focus on the SBM and suppress the comments about other models page 8. They can report these references to the conclusion section if they think that it is usefull althought I do not think it is.
 }
Section 4 now focusses exclusively on existing SBM methods from the literature.
As suggested by Reviewer\#1, in Section~1(`Introduction') we have added more references for a variety
of non-SBM methods, including non-statistical approaches.

\green{
 However they missed the variationnal bayesian estimation method which is a direct competitor to their method
 (S. Gazal  et al. Accuracy of variational estimates for random graph mixture models, Journal of Statistical Computation and
Simulation, 2011). The paper from Bickel, P. and Chen, A. (2010), A nonparametric view of network models and
newman-girvan and other modularities, PNAS, has also some connection, using a profile likelihood which has some similarities with the "collapsed MCMC".
}
Done. The Bickel reference has been added to Section~4(page~10, line~262). And Gazal on line 283.
We have also referenced Gazal in our updated Conclusion, where we question
the claim that MCMC is necessarily unscalable.
We do not intend to argue that MCMC will always be competitive with the best algorithms,
our goal is simply to caution against overly-general claims about MCMC.

\green{
The section 4 named Related probabilistic models should be renamed Related estimation procedures.
}
Done.

\green{
2.2 The two pages about model selection could be shortened because most of the contents is well known. The authors should focus about what they are doing. The explanation about why is too long, not clear and creates some confusion about their own algorithm.
}
Agreed. This section has been rewritten and is shorter.
See our response to Reviewer\#1 above for more details, lines 1099-1106.
% \noindent Done. It's now much shorter.  I might blog about the other stuff that I've just removed.
% We thought our content was newish, but this reviewer says ``most of the contents is well known'' - that's cool.
% I won't have anything useful to say on this topic, at least unless it is combined with the `K!' issue that was discussed in Guelph.

\green{
2.3 I am not convinced by the term "collapsing". The term "collapsibility" has a precise meaning for contingency tables. It is used here in a different way. In this paper the "collapsing" is nothing else than the computation of a marginal distribution, when this marginal can be expressed explicitly. Why using a new term when the term "marginal distribution" which is more precise could be used?
I know that the term collapsing has been already used in one or two papers, but very few (bayesian) statistician have heard about it. The section 3 could be renamed `Marginal distribution of P(x,z,K)'.
}
We have edited the paper to be more careful when introducing the term collapsing for the first time, on line 8.
There are other Bayesian papers that have used ``collapsing'' to mean simply the calculation of the
marginal distribution \cite{LiuCollapsedGibbs,WyseFriel};
a search for ``collapsed Bayesian'' on Google yields many results.
It does appear that the term is already popular in this context,
although we acknowledge the term now has a different meaning from the meaning it has for contingency tables.


\green{
2.4 The authors claim that the proposed algorithm can deal with large networks. However the M3 procedure is of order $N^2$. Therefore it seems that some optimization made for sparse networks is necessary to analyze 10 000 nodes. The authors should not overgeneralize their conclusions and say what happens for a not-sparse 10 000 nodes network.
}
Our algorithm has been optimized to handle sparse networks, see lines~419-425 and lines~460-475.
We have edited our paper to confirm that $N^2$ is the worst case,
and to more carefully justify our claims regarding sparser networks.




\green{
Minor comments

Page 5 the prior on K is a Poisson(1) distribution. What about the case K=0?
}
We had neglected that. Thanks. We now discuss this near the start of Section~3(`Collapsing').
In practice, this cancels out in the posterior as we are only
interested in the posterior mass up to proportionality.

\green{
Page 6 l 13-16. The argument about the correlation between old and new estimate of z is not convincing. Why the reader should believe the authors on this point? In the absence of precise mathematical argument, this sentence should be suppressed.
}
This has been removed.
We might consider it again in a future publication - although perhaps a similar argument (more carefully made) has already appeared in the literature.

\green{
Page 16 l 11. The exact search of the optimal relabeling cannot be done. Instead an heuristic is used. No information is given about the loss between the exact and the heuristic procedures. The reader would like to have some indication about it.
}
More information and discussion has been added in Subsection~5.6(` Label Switching'), lines 544-549 and 570-576.
The issue has not been considered in great detail in the other literature on which our method
is based.
We have calculated the size of the space of all relabellings and shown that it is very large,
ruling out a naive algorithm.
In our experiments, if we take two relabelled states at random, we see that only very
few of the nodes are assigned differently in the two states.
Now, our paper argues that this is suggestive that the heuristic has performed well.
But we do not claim to have proved this.


\green{
Page 21 Table 2. Time to convergence is given for different cases but I have not been able to find any indication about the hardware used.
}
The hardware used is described in section Subsection~5.6(` Label Switching'), line 556/557, and at the start of Section~6(`Evaluation'), lines 584-586.
The same hardware was used for all experiments.

\green{
Page 24 Extensions. The hierarchical extension could be suppressed and the idea kept for a new paper.
}
Agreed. This section, the old Section 8, has now been removed.

\green{
Page 24 l -8 : I do not understand the sentence "It can be meaningful to have clusters that are empty".
}
Agreed.  That sentence has been removed.  Our original intention was to observe that it can be valid for there to be empty clusters.
But that is a very abstract comment, and it is not needed for our paper.
The word `meaningful' was not very helpful.


\subsection{Editor's comments}

\green{
Editor's Comments (provide a point to point response to these comments)
------------------
}

\green{
1. Follow all the editorial guidelines when you prepare the revised
   mns.  (eg abstract in the third person and no statements like this
   paper etc.)

   Re-write the abstract in the third person and without references.
}
Done.

\green{
2. Have the paper proof read and corrected.
}
Done.

% \green{
% 3. Consider recently CSDA published papers that are related in your
   % paper.  http://www.sciencedirect.com/science/journal/01679473
%
   % It is important to related your mns to recent CSDA mns in the area.
   % This will be of great interest to the CSDA readership.
% }
% \{ We'll ignore this :-) \}
\green{

4. Delete the vertical lines from the tables.
}
Done.
\green{
5. Incorporate all footnotes in the main text of the paper (i.e. no
   footnote apart from the first footnote indicating the details of
   the corresponding authors).
}
Done.
\green{
6. Add full stops and commas at the end of equations.
}
Done.






\green{
GUIDELINES FOR PREPARING THE REVISED PAPER

---------------------------------------------------------------------

Please take the following in to account when you prepare the final
version of your paper:
}

\green{
1. Could you please write the abstract in the third person without
   having expressions like "We", "In this paper", "Here", "This work",
   etc.  PLEASE AVOID EQUATIONS IN THE ABSTRACT.
}
Done.
\green{

2. Avoid references in the abstract.  IF THIS IS REALLY NECESSARY,
   then provide complete and abbreviated information.  I.e. (Authors,
   abbr. journal, pages, vol., year).
}
Done.
\green{

3. Do not use vertical lines in tables.
}
Done.

\green{
4. Add the tables at the appropriate place in the paper, i.e. NOT at
   the end.  If you use LATEX, then please incorporate the figures at
   their appropriate place in the paper too.
}
Done.

\green{
5. Add full stops and commas at the end of equations.
}
Done.

\green{
6. The article is written using the CSDA guidelines (see author
   instructions of the journal) and http://www.elsevier.com/locate/csda

7. If you are using Latex, then could you please use the style files
   of the publishers which can be found at
   http://www.elsevier.com/locate/latex/journals/
}
We now use the \verb#elsarticle.cls# style, although further work may be
required to get the right style.

\green{
8. The complete postal address, email, tel. and fax of the
   corresponding author should be shown as a footnote in the first
   page.

   Avoid having any other footnotes.
}
Done.

\green{
9. If you have attachments (software or data sets) that will appear
   as annexes in the electronic version of your mns, then please do
   mention this as a footnote in the first page.
   }
   We have no attachments.
\green{
10. In multiple equations have commas at the end of each eqn and an
    "and" between the last pair.  E.g.

      eqn 1,
      eqn 2,
      eqn 3
     and
     eqn
}
Done.

